Doubly Constrained Fair Clustering

The remarkable attention which fair clustering has received in the last few years has resulted in a significant number of different notions of fairness. Despite the fact that these notions are well-justified, they are often motivated and studied in a disjoint manner where one fairness desideratum is considered exclusively in isolation from the others. This leaves the understanding of the relations between different fairness notions as an important open problem in fair clustering. In this paper, we take the first step in this direction. Specifically, we consider the two most prominent demographic representation fairness notions in clustering: (1) Group Fairness (GF), where the different demographic groups are supposed to have close to population-level representation in each cluster and (2) Diversity in Center Selection (DS), where the selected centers are supposed to have close to population-level representation of each group. We show that given a constant approximation algorithm for one constraint (GF or DS only) we can obtain a constant approximation solution that satisfies both constraints simultaneously. Interestingly, we prove that any given solution that satisfies the GF constraint can always be post-processed at a bounded degradation to the clustering cost to additionally satisfy the DS constraint while the reverse is not true. Furthermore, we show that both GF and DS are incompatible (having an empty feasibility set in the worst case) with a collection of other distance-based fairness notions. Finally, we carry experiments to validate our theoretical findings.

==> Conclusion.tex <==
\section{Conclusion}
\SE{see if there is enough space} 

==> DS_incompatability.tex <==
\subsection{\DS{} Incompatibility} 

Set $k=3$: 
\paragraph{Agnostic} Would have two blue centers and one red. 

\paragraph{\DS{}:} $k_{\text{red}}=2$ and $k_{\text{blue}}=1$. 


The issue is that for Neighborhood and proportionality constraints we need $\frac{n}{k}=\frac{n}{3}=2 \frac{n}{6}$ not $\frac{n}{6}$.   


\begin{fact}
\DS{} constraints and clustering aligned constraints cannot be satisfied simultaneously. 
\end{fact}
\begin{proof}
See Figure \ref{fig:ds_incomptability_3color}. 
\begin{figure}[h!]
  \centering
  \includegraphics[scale=0.5]{Figs/three_communities_DS_violation.png}
   \caption{.}
   \label{fig:ds_incomptability_3color}
\end{figure}

Set $k=3$. From the figure the only feasible clustering-aligned solution is to pick a center from each mass. However, for \DS{} consider the simple setting where $\beta_{\text{blue}},\beta_{\text{red}},\beta_{\text{green}}>0$, this implies that we need to have at least one center from each color. Since the red and green points are only on the rightmost mass, it follows that there will be a mass for which all points have a center which is at best a distance $R$ away. 
\end{proof}

==> Pof_and_incompatability.tex <==
\section{The Price of (Double) Fairness and Incompatibility with Other Distance-Based Fairness Constraints}
\begin{figure}[h!]
  \centering
  \includegraphics[scale=0.4]{Figs/PoF_Taxonomy.png}
   \caption{Figure showing the relation between different constraints. \SE{Update the figure}}
   \label{fig:constraines_relation_ds_gf_agnostic}
\end{figure}
Here we study the degradation in the clustering cost (the price of fairness) that comes from imposing a fairness constraint on the clustering objective as well as the incompatibility between the \DS{} and \GF{} constraints and a family of fairness constraints which we call \emph{clustering-aligned} constraints. 

Before we proceed, we define the following clustering instance: 
\begin{definition}\label{defn:kcommunity} $\ell$-Community Instance: The $\ell$-community instance is a clustering instance where the set of points $\Points$ can be partitioned into $\ell$ communities (subsets) $\{C^{CI}_1,\dots,C^{CI}_{\ell}\}$ of coinciding points (points within the same community are separated by a distance of $0$). Further, the communities are of equal size, i.e. $\forall i \in \ell: |C^{CI}_i|= \frac{n}{\ell}$ . Moreover, the distance between any two points belonging to different communities in the partition is at least $R > 0$. 
\end{definition}
Figure \ref{fig:ci_examples} \SE{include the figure} shows the two examples of $\ell$-community instances. When clustering with a value of $k$, the given a $\ell$-community instance with $k=\ell$ is arguably the most ``natural'' clustering instance where would expect the clustering output to be the communities $\{C^{CI}_1,\dots,C^{CI}_{k}\}$. Further, the fact that all communities have the same population suggests that each community should be a cluster. \SE{maybe talk in the appendix about constraints which are not clustering-aligned}

The following fact clearly holds for any $\ell$-community instance: 
\begin{fact}\label{fact:ci_opt_sol}
If we cluster an $\ell$-community instance with $k=\ell$ then: (1) The set of optimal solutions are $(\stc,\phitc)$ where $\stc$ has exactly one center from each community $\{C^{CI}_1,\dots,C^{CI}_k\}$. Further, points are assigned to a center in the same community. (2) Clustering cost of $(\stc,\phitc)$ is 0. (3) Any solution other than $(\stc,\phitc)$ has a clustering cost of at least $R>0$.  
\end{fact}




\begin{figure}[h!]
  \centering
  \includegraphics[scale=0.4]{two_community_instance.png}
   \caption{In the figure we have $\frac{n}{2}$ blue points that coincide (have distance zero from one another) separated by a distance of $R$ from another set of $\frac{n}{2}$ coinciding red points.}
   \label{fig:gf_unbounded_pof}
\end{figure}

% \begin{definition}
%     Clustering-aligned Constraint:
%     Let $(\stc,\phitc)$ denote a class of solutions of the $k$ Community Instance where $\stc$ is any set of centers that has one point from each subset as the center. $\phitc$ is the assignment function that assigns each point to the closest center. We define Clustering-aligned constraint to be a constraint such that satisfying such a constraint on the $k$ community instance implies clustering problem only has $(\stc,\phitc)$ as feasible solutions.
% \end{definition}


% I.e., $\POF_{c}=\frac{\text{Clustering Cost subject to Constraint $c$}}{\text{Clustering Cost of Agnostic Solution}}$. Note that we are concerned with the price of fairness in the \emph{worst case} throughout this section. 





==> exact_preservation_GF2GFDS.tex <==
\subsection{Exact-Preservation}
We refer to the case where the lower and upper proportionality bounds coincide as the \textbf{exact preservation} case \cite{bercea2018cost}. I.e., in exact preservation we have $\forall h \in \Colors: \beta_h=\alpha_h=r_h$. This implies that (1) For \GF{} we have $|C^h_i|=\rh |C_i| \ \forall i \in S$, (2) For \DS{} we have $\forall h \in \Colors: k_h=\rh k$. This case is clearly restrictive but serves as a good starting point to study how we may satisfy both \GF{} and \DS{} simultaneously.  

Before proceeding into the algorithm we note the following facts and definitions. $\forall h \in \Colors: \rh=\frac{\nh}{n}$. The entire dataset can be considered to be composed of ``atoms'' of each color. Specifically, we are given $n_1,\dots,n_m$ points of each color such that $\sum_{h =1}^m n_h=n$ but there can be common divisors among $n_1,\dots,n_m$. We refer to the ``atomic'' numbers of each color by $n'_1,\dots,n'_m$ and to the size of the atom by $n'=\sum_{h=1}^n n'_h$, clearly $\rh=\frac{n'_h}{n'}$. See the following example for an illustration: 
\paragraph{Example:} 
Consider a dataset which has 3 color ($m=3$) and in the following values $n_1=200,n_2=400$, and $n_3=600$. We have: 
\begin{align*}
    & n_1 \ \ : \ \ n_2 \ \ : \ \ n_3 \\
    & 200 \ \ : \ \ 400 \ \ : \ \ 600 \\ 
    & 1 \ \ : \ \ 2 \ \ : \ \ 3 \\   
\end{align*}
Where we obtained the last line by dividing by all of the common factors and clearly $n'_1=1,n'_2=2,n'_3=3$ and $n'=6$. Further, $r_1=\frac{1}{6},r_2=\frac{1}{3},r_3=\frac{1}{2}$. 

According to the above we have $n=An'$ where $A$ is a positive integer. Further, we also have the following restriction over the choice of centers we can have if we want to satisfy \DS{} at exact preservation:
\begin{fact}\label{fact:kvals_exact_preservation}
To satisfy the \DS{} constraint at exact preservation, then $k=\ell n'$ where $\ell$ is a positive integer. 
\end{fact}
\begin{proof}
By contradiction suppose that this is not the case and that $\ell$ is a positive number but not an integer, then: 
\begin{align*}
    \kh & = \rh k \\ 
    & = \rh (\ell n') \\ 
    & = \rh n' \ell \\  
    & = n'_h \ell \\ 
    & = n'_h \floor{\ell} + n'_h (\ell - \floor{\ell}) 
\end{align*}
Now we show that if $\kh=n'_h \floor{\ell} + n'_h (\ell - \floor{\ell})$ is an integer $\forall h \in \Colors$ then we have a contradiction. To see that, note that the first term $n'_h \floor{\ell}$ is an integer $\forall h \in \Colors$, and therefore $n'_h (\ell - \floor{\ell})$ must be an integer  $\forall h \in \Colors$ to make $\kh$ an integer. However, if $n'_h (\ell - \floor{\ell})$ is an integer $\forall h \in \Colors$ then the numbers $n'_1,n'_2,\dots,n'_m$ are not atomic since we were able to find a common divisor that still leads to integer values which is a contradiction to the definition of $n'_1,n'_2,\dots,n'_m$. This follows since  $\ell$ is not an integer and therefore $(\ell - \floor{\ell}) \in (0,1)$ (must be fractional). 
% however since $\ell$ is not an integer $(\ell - \floor{\ell})$ is not. 
% there must be a color $h$ such that $n'_h (\ell - \floor{\ell})$ is not an integer, otherwise this implies that there is a common divisor between $n'_1,\dots,n'_m$ which contradicts the definition of $n'_1,\dots,n'_m$.
\end{proof}

\begin{fact}\label{fact:gf_kvals_exact_preservation}
To satisfy the \GF{} constraint at exact preservation, then number of active centers $k$ will always satisfy $k\leq A$.  
\end{fact}
\begin{proof}
For a cluster to be fair, then for each active center $i$ we must have $|C^h_i|=\rh |C_i|$. Therefore by definition of the atom numbers $n'_1,\dots,n'_m$ and $n'=\sum_{h=1}^m n'_h$ it follows that $|C_i| \ge n'$. Suppose that $k>A$, then the number of points covered by the centers would be $\sum_{i=1}^k |C_i| \ge k n'> A n'=n$ which is a contradiction. 
\end{proof}


Before we present our result we note the following fact:
\begin{fact}\label{fact:gf_opt_sol_less_centers}
An optimal solution for the \GF{} constraint for the $k$-center problem may have $\bk<k$ many centers.
\end{fact}
\begin{proof}
Consider the Figure \ref{fig:active_vs_nonactive}, if $k=2$, then since we have 4 points and at most only 2 centers, there must be a point will be assigned to a center that is at least a distance of 1. Consider the solution which opens only one center at 2 and assigns all points to it. Clearly this solution satisfies \GF{} and has a cost of 1 which is optimal.  
\end{proof}

\begin{theorem}\label{th:gf_to_gfpds_exact}
For the exact preservation case, given a solution $(\bs,\bphi)$ that satisfies \GF{} for the $k$-center problem with cost $\barf$, then we can obtain a solution $(S,\phi)$ that satisfies both \GF{} and \DS{} constraints simultaneously at a cost of $2\barf$ using Algorithm \ref{alg:exact_pres}. 
\end{theorem}
\begin{proof}
By Fact \ref{fact:gf_opt_sol_less_centers} the solution $(\bs,\bphi)$ has $\bk$ many centers which are possibly less than $k$, i.e. $\bk\leq k$. We note the following fact: 
\begin{fact}\label{fact:gf_sol_properties}
(1) $\forall i \in \bs: |\bar{C}_i|=\ell_i n'$ where $\ell_i$ is a positive integer, (2) $|\bar{C}^h_i|=\ell_i n'_h \ \forall h \in \Colors$, and (3) $\sum_{i \in \bs} \ell_i=A$.  
\end{fact}
\begin{proof}
First, since the solution satisfies the \GF{} constraints, then it must be the case that $\forall i \in \bs:  |\bar{C}^h_i|= \rh  |\bar{C}_i| = \rh \ell_i n'=\ell_i n'_h $. Therefore proving the first statement is sufficient to prove the second. Proving the first statement is done by an argument that is similar to the proof of Fact \ref{fact:kvals_exact_preservation}. By contradiction, suppose that for some $i \in \bs$ we have $|\bar{C}_i|=\ell_i n'$ where is not an $\ell_i$ is not an integer, then
\begin{align*}
    |\bar{C}^h_i| & = \rh |\bar{C}_i|\\ 
    & = \rh (\ell_i n') \\ 
    & = \rh n' \ell_i \\  
    & = n'_h \ell_i \\ 
    & = n'_h \floor{\ell_i} + n'_h (\ell_i - \floor{\ell_i}) 
\end{align*}
If $\ell_i$ is not an integer, then the only way for $|\bar{C}^h_i|$ to be an integer for all $h\in \Colors$ is for $n'_h (\ell_i - \floor{\ell_i})$ to be an integer for all $h\in \Colors$. But if that happens then it negates the definition of $n'_1,\dots,n'_m$. 

The third statement follows since the clusters must cover all of the points. I.e., $n=\sum_{i \in \bs}|C_i|=\sum_{i \in \bs} \ell_i n'$. By dividing by $n'$ we get $A=\sum_{i \in \bs} \ell_i$.  
\end{proof}
The above fact indicates that the clusters in the given solution $(\bs,\bphi)$ each consist of integral multiples of the atoms. 

Algorithm \ref{alg:exact_pres} generates the solution $(S,\phi)$ which satisfies both constraints with a cost of at most $2\barf$. For now we ignore the analysis of the cost $f$ and only focus on showing that the output would satisfy both the \GF{} and \DS{} constraints. 

Lines (3-10) in Algorithm \ref{alg:exact_pres} update the cluster centers to other points within the same cluster but of a possibly different color. Since the cluster already satisfy the \GF{} constraints and that we always update the assignment of entire cluster to the same center, it follows that the new clusters in solution $S$ satisfy the \GF{} constraint. 

Since $\bk\leq k$ and $\sum_{h=1}^m \kh =k$ at the end of line (10) there may still be colors which have not been assigned enough centers, i.e. $q_h < \kh$. The set $\Colors'$ is the set of colors which have not received enough centers. Since there are centers for which $\ell_i>1$ (more than one atom) we use them to open new centers and assign atoms to them. In lines (12-25) each color which still does not have $\kh$ centers is given more centers from a cluster with multiple atoms and assigned atoms. Since entire atoms which share the same cluster are assigned to the same new center the \GF{} constraint is satisfied. Further, by Fact \ref{fact:gf_kvals_exact_preservation} we have $k\leq A$ and by part (3) of Fact \ref{fact:gf_sol_properties} there must be enough atoms to assign to each center. 

To upper bound the clustering cost $f$ we make the following observation: 
\begin{observation}
In Algorithm \ref{alg:exact_pres} for any point $j \in \Points$ the final assigned center of the point is always another point in the same original cluster. 
\end{observation}
From the above observation it follows that $\forall j \in \Points: d(j,\phi(j)) \leq d(j,\bphi(j))+d(\bphi(j),\phi(j)) \leq \barf + \barf =2 \barf$. 
\end{proof}


\begin{algorithm}[h!] %https://tex.stackexchange.com/questions/56871/how-to-format-for-loop-for-printing-a-pseudo-code-listing 
    \caption{\textsc{Exact Preservation: Post-processing \GF{} Solution to Satisfy \GF{}+\DS{}}}\label{alg:exact_pres}
    \begin{algorithmic}[1]
    \STATE \textbf{Input}: Points $\Points$, Color membership function $\chi:\Points \xrightarrow{} \Colors$, Solution $(\bs,\bphi)$ with clusters $\{\bar{C}_i,\dots,\bar{C}_{\bk}\}$ satisfying the \GF{} constraints with $|\bs|=\bk \leq k$.  
    \STATE \textbf{Output}: Solution $(S,\phi)$ satisfying the \GF{} and \DS{} constraints simultaneously.
    \item[] % skip line (unnumbered) 
    \STATE Initialize $q_h=0 \ \forall h \in \Colors \ $. //$q_h$ is a counter for the number of centers color $h$ has.
         \FOR{$i: 1 \ \text{to} \   \bk$} 
              \STATE Pick a color $h$ such that $q_h < \kh$.
              \STATE Choose a point $i'$ of color $h$ in cluster $\bar{C}_i$. 
              \STATE Set $S=S\cup \{i'\}$ and set $\forall j \in \bar{C}_i: \phi(j)=i' \ $ \COMMENT{Set $i'$ as a center and assign it all of cluster $\bar{C}_i$, therefore $C_i=\bar{C}_i$.} 
              \STATE Update $q_h = q_h+1$
              \STATE Update $\ell_i = \ell_i -1$
      \ENDFOR
    \STATE Set $\Colors' = \{h \in \Colors: q_h <\kh\} \ $ \COMMENT{$\Colors'$ is the set of colors that still don't have many $\kh$ centers.}
    %\STATE Set $\cali=\{i \in [k]: \ell_i>1\}$  
        \FOR{$h \in \Colors' \ $} 
             \FOR{$i: 1 \ \text{to} \   \bk$}
                \IF{$\ell_i> 0 $} 
                    \STATE  $\Delta = \min\{k_h -q_h,  \ell_i\}$
                    \IF{$\Delta >0 $}
                         \STATE Choose $\Delta$ many points $S'$ from cluster $C_i$ all of color $h$. Further, $S'\cap S=\{\} \ $  \COMMENT{The $S'$ points were not set as centers in the new solution.} 
                         \STATE Update $S=S\cup S'$
                         \STATE Update the assignment $\phi$: For each center in $S'$ assign it $n'_{\Tilde{h}}$ from each color $\Tilde{h}$ where all of the $n'_{\Tilde{h}}$ points of each color belong to cluster $C_i$. 
                         \STATE Update $q_h = q_h + \Delta$ 
                         \STATE Update $\ell_i =\ell_i -\Delta$
                    \ENDIF
                \ENDIF
            \ENDFOR
      \ENDFOR
\end{algorithmic}
\end{algorithm}



\begin{corollary}
For the exact preservation case, given an $\alpha_{\GF}$-approximation algorithm for \GF{}, then we can have a $2\alpha_{\GF}$-approximation algorithm for \GF{} and \DS{} simultaneously. 
\end{corollary}
\begin{proof}
Using the previous theorem (Theorem \ref{th:gf_to_gfpds_exact}) the solution $(\bs,\bphi)$ has a cost of $\barf \leq \alpha_{\GF} \OPT_{\GF}$. The post-processed solution that satisfies \GF{} and \DS{} simultaneously has a cost of $f \leq 2 \barf \leq 2 \alpha_{\GF} \OPT_{\GF} \leq 2 \alpha_{\GF} \OPT_{\GF+\DS}$. The last inequality follows because $\OPT_{\GF} \leq \OPT_{\GF+\DS}$ which is the case since both problems minimize the same objective, however by definition the constraint set of $\GF+\DS$ is a subset of the constraint set of $\GF$.   
\end{proof}

\begin{figure}[h!]
  \centering
  \includegraphics[scale=0.5]{gf_to_ds_fig.png}
   \caption{Post-processing a solution that satisfies \GF{} to satisfy both \GF{} and \DS{} simultaneously.}
   \label{fig:gf_to_ds}
\end{figure}

==> general_proportion_bounds.tex <==
\newpage 
\subsection{General Proportion Bounds: $k$-center} 
Here we are dealing with general bounds but as always we have $\beta_h >0 \ , \forall h \in \Colors$. Also, the value of $k$ and the bounds $\{ \alpha_h,\beta_h\}_{h \in \Colors}$ have a valid assignment. We have a solution $(\bs,\bphi)$ of cost $\barf$ that satisfies the \GF{} constraints and we want to make it satisfy \GF{} and \DS{} simultaneously. 

Since the value of $k$ and the bounds $\{ \alpha_h,\beta_h\}_{h \in \Colors}$ have a valid assignment we simply start with color $h_1$ go to the first cluster and pick a point of color $h_1$ as center and then go the next cluster and pick a point of color $h_1$ and so on until we have at least $\beta_{h_1} k$ and then we go to color $h_2$ and do the same. If new total centers picked is less than $\bk$, then we pick more points of colors $h$ that have not reached the upper bound $\alpha_h k$ and so on until we cover of $\bk$ centers. \SE{This should be more formal and clear}.  


\begin{algorithm}[h!] %https://tex.stackexchange.com/questions/56871/how-to-format-for-loop-for-printing-a-pseudo-code-listing 
    \caption{\textsc{Post-Process\GF{}To\GFPDS{}}}\label{alg:general_gfTogfds_kcenter}
    \begin{algorithmic}[1]
    \STATE \textbf{Input}: Points $\Points$, Color membership function $\chi:\Points \xrightarrow{} \Colors$, Solution $(\bs,\bphi)$ with clusters $\{C_i,\dots,C_{\bk}\}$ satisfying the \GF{} constraints with $|\bs|=\bk \leq k$.  
    \STATE \textbf{Output}: Solution $(S,\phi)$ satisfying the \GF{} and \DS{} constraints simultaneously.
    \item[] % skip line (unnumbered) 
%\STATE Set $(S',\phi')=(\bs,\bphi)$ \COMMENT{this implies that $k'=|S'|=|\bk|=\bk$.}
\STATE Initialize: $S'=\{\}$, $\forall h \in \Colors: q_h=0$, $\forall i \in [\bk]: Q_i=\{\}$.
\FOR{$i=1$ to $\bk$} 
    \IF{$\exists h \in \Colors: q_h < \alpha_h k$} 
        \STATE Let $h'$ be a color such that $q_{h'} < \beta_{h'} k$, if no such point exists, then set pick ${h'}$ such that $q_{h'}+1\leq \alpha_{h'} k$. 
        \STATE Pick a point $j_{h'}$ of color ${h'}$ in cluster $\bar{C}_i$
        \STATE Set $Q_i = Q_i \cup \{j_{h'}\}$. 
        \STATE Update $q_h=q_h+1$. 
    \ENDIF
\ENDFOR 
\WHILE{$\exists h  \in \Colors: q_h <\beta_h k$}
        \STATE Pick a random center $i \in [\bk]$ with cluster $\bar{C}_i$. 
        \STATE Let $h'$ be a color such that $q_{h'} < \beta_{h'} k$, if no such point exists, then set pick ${h'}$ such that $q_{h'}+1\leq \alpha_{h'} k$. 
        \STATE Pick a point $j_{h'}$ of color ${h'}$ in cluster $\bar{C}_i$
        \STATE Set $Q_i = Q_i \cup \{j_{h'}\}$. 
        \STATE Update $q_h=q_h+1$. 
\ENDWHILE
\FOR{$i=1$ to $\bk$} 
\STATE $\phi_i =$ \textsc{Divide}($\bar{C}_i,Q_i,\{\beta_h,\alpha_h\}_{h \in \Colors},0$).  
\ENDFOR 
\STATE Set $S =\cup_{i \in \bk} Q_i$ and construct $\phi$ from $(S_i, \phi_i)$. \SE{More clear here}
\end{algorithmic}
\end{algorithm}






% Before we show the main result. We have the following lemma: 
% \begin{lemma}\label{lemma:divide}
% Given a cluster $\bar{C}_i$ that satisfies the \GF{} constraints and a subset of $t$ points in the cluster $Q_i$ ($Q_i \subset \bar{C}_i$). Then clustering $(Q_i,\phi)$ where $\phi_i =$ \textsc{Divide}($\bar{C}_i,Q_i$) satisfies the \GF{} constraints at an additive violation of 2 \SE{and all of the centers are active}. 
% \end{lemma}
% \begin{proof}
% We begin with the following fact: 
% \begin{fact}
% $LP(\bar{C}_i,Q_i)$ is feasible. 
% \end{fact}
% \begin{proof}
% We show that the LP is feasible by showing a set of possible values for $x_{cj}$ that satisfy all of the constraints of (\ref{lp:divide_lp}). Let $z_{ij}$ be the assignment in cluster $\bar{C}_i$ to the original center $i$, then set $x_{cj} = \frac{z_{ij}}{t}$. Note that $z_{ij}$ satisfies the \GF{} constraints. 

% For constraint \ref{constraint:equal_split} we have $\forall c \in Q_i: \sum_{j \in \bar{C}_i} x_{c j} = \sum_{j \in \bar{C}_i} \frac{z_{i j}}{t} =\frac{\bar{C}_i}{t}$ and therefore holds. For constraint \ref{constraint:GF_constraint}, we have: 
% \begin{align}
%     \forall h \in \Colors, \forall c \in Q_i: & \beta_h \sum_{j \in \bar{C}_i} x_{c j}  \leq  \sum_{j \in \bar{C}_i \cap \Points^h} x_{c j} \leq \alpha_h \sum_{j \in C'_{t}} x_{c j} 
% \end{align}
% since the bounds for a given color for $z_{i j}$ and $x_{c j}=z_{i j}/t$. Moreover, constraint  \ref{constraint:assigned} holds since $\sum_{c \in Q_i} x_{cj} = \sum_{c \in Q_i} \frac{z_{ij}}{t} = \sum_{c \in Q_i} \frac{1}{t}=1$. The last constraint clearly holds.  
% \end{proof}
% Since $LP(\bar{C}_i,Q_i)$ is feasible, the solution we find can be plugged into MaxFlowGF($\bold{x}^*,\bar{C}_i,Q_i,\{\beta_h,\alpha_h\}$) and we get the guarantees from \cite{bercea2018cost}. 
% \end{proof}

Now we state the main theorem: 
\begin{theorem}\label{th:gf_to_gfds_general_bounds}
If we have a solution $(\bs,\bphi)$ of cost $\barf$ that satisfies the \GF{} constraints where the number of non-empty clusters is $|\bs|=\bk=k$, then we can obtain a solution $(S,\phi)$ satisfy the \GF{} at an additive violation of 2 and \DS{} constraints simultaneously with cost $f\leq 2\barf$. 
\end{theorem}
\begin{proof}
First we note the following fact: 
\begin{fact}
Every cluster in $(\bs,\bphi)$  has at least one point from each color. 
\end{fact}
\begin{proof}
This holds, since given a center $i \in \bs$ we have $|\bar{C}_{i}|>0$ and therefore $\forall h \in \Colors: |\bar{C}^{h}_i| \ge \beta_h |\bar{C}_{i}|>0$ and therefore $|\bar{C}^{h}_i|\ge 1$ since $|\bar{C}^{h}_i|$ is an integer.  
\end{proof}
The above fact implies that the loop from lines (4-11) is always able to add a center for a color. 

By Lemma \ref{lemma:divide} for \textsc{Divide} the new centers $\mathcal{Q}=\cup_{i \in [\bk] } Q_i$ are all active (guarantee 2 of \textsc{Divide}) and by the center selection method we have $\forall h \in \Colors: \beta_h k\leq |\mathcal{Q} \cap \Points^h| \leq \alpha_h k$. Further, each cluster satisfies the \GF{} constraints at an additive violation of $2$ since we have $\rhp=0$ here (guarantee 1 of \textsc{Divide}). Finally, the clustering cost is at most $f\leq 2 \barf$ (guarantee 3 of \textsc{Divide}). 
\end{proof}




\begin{corollary}
Given an $\alpha_{\GF}$-approximation algorithm for \GF{}, then we can have a $2\alpha_{\GF}$-approximation algorithm that satisfies \GF{} at an additive violation of $2$ and \DS{} simultaneously. 
\end{corollary}
\begin{proof}
Using the previous theorem (Theorem \ref{th:gf_to_gfds_general_bounds}) the solution $(\bs,\bphi)$ has a cost of $\barf \leq \alpha_{\GF} \OPT_{\GF}$. The post-processed solution that satisfies \GF{} at an additive violation of 2 and \DS{} simultaneously at a cost of $f \leq 2 \barf \leq 2 \alpha_{\GF} \OPT_{\GF} \leq 2 \alpha_{\GF} \OPT_{\GF+\DS}$. The last inequality follows because $\OPT_{\GF} \leq \OPT_{\GF+\DS}$ which is the case since both problems minimize the same objective, however by definition the constraint set of $\GF+\DS$ is a subset of the constraint set of $\GF$.   
\end{proof}


\paragraph{Remark:} If the given \GF{} solution has the number of cluster $\bk=k$, then the output will have an additive violation of zero, i.e. satisfy the \GF{} constraints exactly. This would happen \textsc{Divide} would always receive $Q_i$ with $|Q_i|=1$ and therefore we can use the guarantee of \textsc{Divide} for the special case of $|Q|=1$. 

% \SE{END END END END END END}
% We start with the theorem for the special case where $|\bs|=\bk=k$. 

% \SE{make this a remark}
% \begin{theorem}
% If we have a solution $(\bs,\bphi)$ of cost $\barf$ that satisfies the \GF{} constraints where the number of non-empty clusters is $|\bs|=\bk=k$, then we can obtain a solution $(S,\phi)$ satisfy the \GF{} and \DS{} constraints simultaneously with cost $f\leq 2\barf$. 
% \end{theorem}
% \begin{proof}
% \begin{fact}
% Every cluster in $(\bs,\bphi)$  has at least one point from each color. 
% \end{fact}
% \begin{proof}
% This holds, since given a center $i \in \bs$ we have $|\bar{C}_{i}|>0$ and therefore $\forall h \in \Colors: |\bar{C}^{h}_i| \ge \beta_h |\bar{C}_{i}|>0$ and therefore $|\bar{C}^{h}_i|\ge 1$ since $|\bar{C}^{h}_i|$ is an integer.  
% \end{proof}

% \begin{fact}
% For any given cluster $\bar{C}_{i}$ of radius $R_i$ if the center $i$ is updated to another point $i'$ within the cluster ($i' \in \bar{C}_{i}$), then (1) the new radius of the cluster is $R'_i \leq 2 R_i$ and (2) the cluster still satisfies the \GF{} constraints.
% \end{fact}
% \begin{proof}
% The second statement follows immediately since the points within the cluster did not change. The first follows since $\forall j \in \bar{C}_{i}: d(j,i') \leq d(j,i)+d(i,i') \leq 2 R_i$.
% \end{proof}


% \end{proof} 
% \SE{END: make this a remark}

==> incompatibility.tex <==
\subsection{Incompatibility with Other Fairness Constraints}\label{sec:incompatibility}
We note that the results of this section do not take into account the clustering cost and are based only on the feasibility set. That is, we consider more than one constraints simultaneously and see if the feasibility set is empty or not. Two constraints are considered \emph{incompatible} if the intersection of their feasible sets is empty. In some cases we also consider solution that could have violations to the constraints. We start by defining a family of distance-based fairness constraints and show that two constraints that were already introduced in the literature belong to this family.  



\SE{We also study constraints between \GF{} and proportionally fair clustering constraint in the appendix.}

% \begin{definition}\label{defn:kcommunity}
%    $k$ Community Instance: 
%   we define $k$ Community Instance to be an instances of clustering problem where we have $k$ subsets of points. Points within the same subset are separated by a distance of $0$. Points from different subsets are separated by $R > 0$. And the size of each subset is $\frac{n}{k}$.
% \end{definition}



\begin{definition} \label{defn:clustering_aligned}
    Clustering-aligned Constraints: \SE{changed to relaxed}
    Given the $\ell$-community instance, a constraint is clustering-aligned if the only feasible $\alpha$-relaxed solution for finite $\alpha$ when $k=\ell$ is a member of the class $(\stc,\phitc)$.   
\end{definition}
% Let $(\stc,\phitc)$ denote a class of solutions of the $k$ Community Instance where $\stc$ is any set of centers that has one point from each subset as the center. $\phitc$ is the assignment function that assigns each point to the closest center. We define Clustering-aligned constraint to be a constraint such that satisfying such a constraint on the $k$ community instance implies clustering problem only has $(\stc,\phitc)$ as feasible solutions.


\begin{definition}\label{defn:neighor_radius}
Neighborhood Radius \cite{jung2019center}:
For a given set of points $\Points$ to cluster and a given number of centers $k$, the Neighborhood Radius of a point $j$ is the minimum radius $r$ such that at least $|C|/k$ of the points in $\Points$ are within distance $r$ of $j$: $ \text{NR}_{C,k}(j)=\min\{r : |B_r(j) \cap C| \geq |C|/k \}$,where $B_r(j)$ is the closed ball of radius $r$ around $j$. 
\end{definition}


%\begin{definition}
%Fairness in Your Neighborhood Constraint\cite{jung2019center}:
%For a chosen set of centers $S$, the maximum ratio between the distance to any center and Neighborhood Radius %over all points in $\Points$ is:
%\begin{align*}
%    \alpha_{\Points,k}(S)=\max_{j \in \Points}\frac{d(j, S)}{\text{NR}_{\Points,k}(j)}
%\end{align*}
%\end{definition}

%We say that a solution $S$ of an instance of clustering problem $(C, k)$ achieves $\alpha$-fairness if $\alpha_{C,k}(S) \leq \alpha$.


\begin{definition}
Fairness in Your Neighborhood Constraint\cite{jung2019center}:
For a given set of points $\Points$ with metric $d(.,.)$, a clustering is $\alpha$ fair if for all $j \in \Points$, $d(j, S) \leq \alpha \cdot \text{NR}_{\Points,k}(j)$.
\end{definition}



\begin{proposition}
Fairness in Your Neighborhood Constraint is clustering-aligned. 
\end{proposition}
\begin{proof}
%\SE{TO DO.}
%\SE{1-show that $\text{NR}_{C,k}(i)=0 \ \forall i \in \Points$. 2-$(\stc,\phitc)$ makes $d(i,\phitc)=\text{NR}_{C,k}(i)=0 $. 3-Any other solution would have $\exists i \in \Points: d(i,\phitc) > \text{NR}_{C,k}(i)$.}
%\SE{Should be for arbitrary $k$}
Consider a clustering problem on the $\ell$-community instance with $k=\ell$. By Definitions \ref{defn:kcommunity} and Definition \ref{defn:neighor_radius},  for any point $i \in \Points$, its neighborhood radius is $\text{NR}_{C,k}(i)=\min\{r : |B_r(i) \cap C| \geq |C|/k\} = 0$.
This is because each point is in one of the $l$ subset, and by definition, the subset is of size $\frac{n}{l}=\frac{n}{k}$, and points in the same subset are separated by a distance $0$. 

If a solution on a $\ell$-community instance $(S, \phi)$ satisfies clustering-aligned constraint, then it is in the set of solutions $(\stc,\phitc)$. For any point $i \in \Points$, because $S$ contains a center in the community where $i$ is, $d(i, S)=0$. Note this is true for any $(S, \phi)$ in the set of solutions  $(\stc,\phitc)$, which means any solution $(S, \phi)$ satisfying clustering-aligned constraint has $d(i, S)=0$.

By definition of $\alpha$-fairness, this means on a $\ell$-community instance, any clustering-aligned solution is $\alpha$-fair with $\alpha=1$. This is because for any $(S, \phi) \in (\stc,\phitc)$, $\alpha_{C,k}(S)=\max_{i \in C}\frac{d(i,S)}{\text{NR}_{C,k}(i)} = \frac{0}{0} = 1$.


In any solution that is not clustering-aligned, there is at least a point which is assigned to a center not in the point's own community. Thus for such a solution $(S, \phi)$, there exist $i \in \Points$, $d(i, S)=R$. Thus for $(S, \phi) \notin (\stc,\phitc)$, $\alpha_{C,k}(S)=\max_{i \in C}\frac{d(i, S)}{\text{NR}_{C,2}(i)} = \frac{R}{0} = \infty$. Thus $\alpha=\infty$ for solutions not in $(\stc,\phitc)$.

This shows that a solution that achieves $\alpha$-fairness for a finite $\alpha$ must be a solution from the set of solutions $(\stc,\phitc)$, thus must satisfies clustering-aligned constraint.
\end{proof}



\begin{definition}\label{defn:socially_fair}
Socially Fair \cite{abbasi2020fair,ghadiri2021socially}: for a clustering problem with center budget $k$ on points $\Points$ which are from $|\Colors|$ groups and $\cup_{h \in \Colors} C^{h}=\Points$, a Socially Fair clustering minimizes the maximum average clustering cost across all groups: $\displaystyle \min_{S: |S|\leq k, \phi} \ \max_{h \in \Colors}\Big( \sum_{j \in C^{h}} d^p(j,\phi(j)) \Big)^{1/p}$.
\end{definition}Note that Socially Fair does not optimize over assignment functions because it assumes assignment follows optimal rule: a point is assigned to the cluster center closest to it.

\begin{definition}\label{defn:alpha_socially_fair}
An $\alpha$-Socially Fair solution to a clustering problem is a solution that achieves $\alpha$ multiplicative approximation in optimization objective to optimal Socially Fair solution. 
\end{definition}

This definition allows us to bound the clustering cost of an $\alpha$-Socially Fair solution $(S_{\alpha}, \phi_{\alpha})$ as:

$\displaystyle
    \max_{h \in \Colors}\Big( \sum_{j \in C^{h}} d^p(j,\phi_{\alpha}(j)) \Big)^{1/p}\leq   \alpha \min_{S: |S|\leq k} \max_{h \in \Colors}\Big( \sum_{j \in C^{h}} d^p(j,\phi(j)) \Big)^{1/p}.
$




\begin{fact}
On a $\ell$-community instance, a Socially Fair clustering solution satisfies clustering-aligned constraint.
\end{fact}


\begin{proof}
Denote optimal solution to the a Socially Fair clustering problem as $\text{OPT}_{SF}$. By definition,
\begin{align*}
\text{OPT}_{SF} = \min_{S: |S|\leq k} \max_{h \in \Colors}\Big( \sum_{j \in C^{h}} d^p(j,\phi(j)) \Big)^{1/p}.
\end{align*}

We can formulate a problem that aims to find an $\alpha$-Socially Fair solution as a constrained optimization problem. We use a dummy objective function $f$. The constraint can be set up as requiring maximum clustering costs across all colors to be upper-bounded by $\alpha$ times that of the optimal Socially Fair solution $\text{OPT}_{SF}$. 

The constrained program can be set up as below:
\begin{align*}
    &\min_{S: |S|\leq k} f \\ 
    &\text{s.t.  }\max_{h \in \Colors} \Big( \sum_{j \in C^{h}} d^p(j,\phi(j)) \Big)^{1/p} \leq \alpha \text{OPT}_{SF}
\end{align*}

For a clustering problem with budget $k$ on the $k$ Community Instance, in a solution $(S, \phi)$ that has one center in each subset, $d(j,\phi(j))=0$ for each point $j \in \Points$. Thus this solution has clustering cost for each color $h$ as $\Big( \sum_{j \in C^{h}} d^p(j,\phi(j)) \Big)^{1/p}=0$. Since $\text{OPT}_{SF}$ is upper bounded by cost of this solution, $\text{OPT}_{SF}=0$. 


Thus on the $k$ Community Instance, feasible solutions to the $\alpha$-Socially Fair problem have $ \max_{h \in \Colors} \Big( \sum_{j \in C^{h}} d^p(j,\phi(j)) \Big)^{1/p} =0$. We now show $(\stc,\phitc)$ is the only set of solutions that have $\max_{h \in \Colors} \Big( \sum_{j \in C^{h}} d^p(j,\phi(j)) \Big)^{1/p} =0$. Thus will be the only feasible solutions. 

For any solution $(S, \phi)$ that is not in $(\stc,\phitc)$, there must be a point assigned to a center that is not in its own community. For such a point $d(j, \phi(j))=R$. Thus 
$ \max_{h \in \Colors} \Big( \sum_{j \in C^{h}} d^p(j,\phi(j)) \Big)^{1/p} \geq R$. And thus any solution that is not in $(\stc,\phitc)$ is not feasible. 

For any solution $(S, \phi)$ that is in the set $(\stc,\phitc)$, its cost $ \max_{h \in \Colors} \Big( \sum_{j \in C^{h}} d^p(j,\phi(j)) \Big)^{1/p} =0$ for $d(j, \phi(j))=0$ for each $j$. Therefore a feasible solution that is socially fair must be clustering-aligned.
\end{proof}




\begin{theorem}
In general, it is impossible to find a solution that satisfies both a clustering-aligned constraint and \DS{} simultaneously. 
\end{theorem}

%\begin{figure}[h!]
%  \centering
%  \includegraphics[scale=0.5]{Figs/three_communities_DS_violation.png}
%   \caption{.}
%   \label{fig:ds_incomptability_3color}
%\end{figure}


\begin{figure}[h!]
  \centering
  \includegraphics[scale=0.4]{Figs/l_community_ds.png }
   \caption{A $l$ community instance to show incompatibility with \DS{}.}
   \label{fig:l_community_ds}
\end{figure}


\begin{proof}
    Consider a case of the $\ell$-community instance where the first $\ell-1$ communities consist of points of only one color. And the last community contains $\frac{n}{2\ell}$ points of each color. In this $\ell$-community instance, as shown in Figure \ref{fig:l_community_for_odd_k}, $\ell-1$ of the subsets contain only points of blue color. The last subset contains $\frac{n}{2l}$ green points and $\frac{n}{2l}$ red points. On this instance, a clustering solution of $k=l$ that satisfies clustering-aligned constraint picks a center from each community. However, satisfying \DS{} with $\beta_{\text{blue}},\beta_{\text{red}},\beta_{\text{green}}>0$ requires a center of each color be picked. Thus a clustering-aligned solution does not satisfy \DS{} because it will only pick one point from the right most subset as a center. Thus either green points or red points will not appear in the set of centers.

    
    On the other hand, since a solution satisfying \DS{} has at least one center of each color, it will contain two centers, one green, one red chosen from the right most subset. And there are $k-2$ centers allocated to the $k-1$ communities on the left. By pigeon hole principle, one of the communities will have no center allocated. All points in this subset are then assigned to a center in a nearby community, violating clustering-aligned constraint.
\end{proof}

\begin{theorem}\label{thm:cannot_exact_satisfy_CA_DS}
In general, it is impossible to find a solution that satisfies both a clustering-aligned constraint and \GF{} simultaneously even if we allow an additive violation of $\Omega(\frac{n}{k})$ to the \GF{} constraint.
\end{theorem}

%\begin{figure}[h!]
%  \centering
%  \includegraphics[scale=0.5]{two_community_instance.png }
%   \caption{The two community instance.}
%   \label{fig:two_community}
%\end{figure}

\begin{figure}[h!]
  \centering
  \includegraphics[scale=0.4]{Figs/l_community_even_k.png }
   \caption{A $l$-community instance to show incompatibility with \GF{} when $k$ is even.}
   \label{fig:l_community_for_even_k}
\end{figure}

\begin{figure}[h!]
  \centering
  \includegraphics[scale=0.4]{Figs/l_community_odd_k.png }
   \caption{A $l$-community instance to show incompatibility with \GF{} when $k$ is odd.}
   \label{fig:l_community_for_odd_k}
\end{figure}


\begin{proof}
Consider the case where $k \ge 2$ is even and refer to Figure \ref{fig:l_community_for_even_k} where we have $\ell=k$ communities that alternate from red to blue color. Further, by Fact \ref{fact:ci_opt_sol} and Definition \ref{defn:clustering_aligned}, a clustering-aligned solution has a clustering cost of $0$ and would have $k$ centers, one center in each community, and the solution assigns each point to its closest center. 

If we set the lower and upper proportion bounds to $\frac{1}{2}$ for both colors, then to satisfy \GF{} each cluster should have both red and blue points. There must exists a cluster $C_i$ of size $|C_i|\ge \frac{n}{k}$, it follows that to satisfy the \GF{} constraints at an additive violation of $\rho$, then $|C^{\text{blue}}_i|\ge \frac{1}{2}|C_i|-\rho = \frac{n}{2k}-\rho$ and similarly we would have $|C^{\text{red}}_i|\ge \frac{n}{2k}-\rho$. By setting $\rho=\frac{n}{2k}-\epsilon$ for some constant $\epsilon > 0$, then we have $|C^{\text{blue}}_i|,|C^{\text{red}}_i|>0$. This implies that a point will be assigned to a center at a distance $R>0$ and therefore violating the clustering-aligned constraint. 

For a value of $k$ that is odd, see the example  Figure \ref{fig:l_community_for_odd_k}. Here instead the last community has the same number of red and blue points. We call the cluster whose center is in the last community $C_{\text{last}}$. By the same argument as the even $k$ case, a clustering-aligned solution has a clustering cost of $0$ and would have $k$ centers, one center in each community, and the solution assigns each point to its closest center.

We still set the lower and upper proportion bounds to $\frac{1}{2}$ for both colors. If $|C_{\text{last}}| \neq \frac{n}{k}$, then there are points assigned to the center of $C_{\text{last}}$ from other communities incurring cost $R>0$ or points in the last community are assigned to other centers at distance $R >0$. In both cases clustering-aligned constraint is violated. If  $|C_{\text{last}}| = \frac{n}{k}$, then in the remaining $k-1$ communities with total of $n-\frac{n}{k}$ points, $k-1$ centers are chosen. A solution satisfying \GF{} has one cluster $C_i$ with at least $\frac{1}{k-1}\left(n-\frac{n}{k}\right) = \frac{n}{k}$ points. Then we follow the same argument as in the even $k$ case. That is, to satisfy \GF{} with $\rho$ additive violation on the $C_i$, $|C^{\text{blue}}_i|\ge \frac{1}{2}|C_i|-\rho = \frac{n}{2k}-\rho$, $|C^{\text{red}}_i|\ge \frac{n}{2k}-\rho$, with $\rho=\frac{n}{2k}-\epsilon$ for some constant $\epsilon > 0$, at least a point will be assigned to center at distance $R>0$ and clustering-aligned is violated.



%The proof would present the two community instance as an example and then show that it's impossible to satisfy both a clustering-aligned and \GF{} simultaneously. Therefore, in general it is impossible to satisfy both. 

%Consider a case of the $k$ Community Instance where $k=2$. We will call this case the Two Community Instance. In the Two Community Instance, as shown in Figure \ref{fig:two_community}, the two subsets each contain only points of one color. The left subset contains $\frac{n}{2}$ blue points, and the right subset contains $\frac{n}{2}$ red points. On this instance, a clustering solution for $k=2$ that satisfies clustering-aligned constraint will have one left center of one color and one right center of the other color. By definition, a solution satisfying clustering aligned constraint will assign each point to its closest center. Therefore, all blue points will be assigned to the blue center, and similarly for all red points. Thus the two clusters formed will each contain points of one single color. To satisfy \GF{} on the Two Community Instance, a solution should form two clusters, each of size $\frac{n}{2}$, of which $\frac{n}{4}$ should be blue and $\frac{n}{4}$ should be red. Since in the solution that satisfies clustering-aligned constraint, each cluster only contains one color, it does not satisfy \GF{}. 

%Similarly, consider a solution that satisfies \GF{} on the Two Community Instance. If the solution has two centers of the same color, it is violating the clustering aligned constraint. 

%Consider the solution which has two centers, one blue and one red. In the cluster with blue center, there are $\frac{n}{4}$ red points which are assigned to the blue center from the red community. Those $\frac{n}{4}$ red points are not assigned to the red center which is closest to them. Therefore clustering aligned constraint is not satisfied.
\end{proof}









\begin{figure}[h!]
  \centering
  \includegraphics[scale=0.4]{constraints_clust_aligned.png}
   \caption{}
   \label{fig:constraints_clust_aligned}
\end{figure}





==> recursive_solution_non_exact_preservation_GF2GFDS.tex <==
\subsection{Recursive Solution NOT BEST IGNORE: General Case Preservation \textcolor{red}{\textbf{(PROOF SKETCH)}}}  
\SE{This is the old version which breaks clusters recursively and requires an assumption on the minimum lower bound $\beta_h \ge \frac{8(k-1)}{n}$}.  


\begin{algorithm}[h!] %https://tex.stackexchange.com/questions/56871/how-to-format-for-loop-for-printing-a-pseudo-code-listing 
    \caption{\textsc{Post-Process\GF{}To\GFPDS{}}}\label{alg:recursive_general_gfTogfds_kcenter}
    \begin{algorithmic}[1]
    \STATE \textbf{Input}: Points $\Points$, Color membership function $\chi:\Points \xrightarrow{} \Colors$, Solution $(\bs,\bphi)$ with clusters $\{C_i,\dots,C_{\bk}\}$ satisfying the \GF{} constraints with $|\bs|=\bk \leq k$.  
    \STATE \textbf{Output}: Solution $(S,\phi)$ satisfying the \GF{} and \DS{} constraints simultaneously.
    \item[] % skip line (unnumbered) 
\STATE Set $(S',\phi')=(\bs,\bphi)$ \COMMENT{this implies that $k'=|S'|=|\bk|=\bk$.}
\STATE Initialize a number $s_i=1 \ , \forall i \in [\bk]$. \COMMENT{$s_i$ is the number of division cluster $i$ will have.}
\FOR{$t=1$ to $(k-\bk)$} 
      \STATE Find $\ell = \argmax_{\ell' \in [\bk]} \frac{|C_{\ell'}|}{s_{\ell'}}$
      \STATE Update $s_{\ell}=s_{\ell}+1$
\ENDFOR

\FOR{$t=1$ to $(k-\bk)$} 
    \IF{$s_t>2$} 
        \STATE $(\{c_{1},\dots,c_{s_t}\},\phi_t) =$ \textsc{Divide}($C_t,s_t$). 
        \STATE Update the set of centers: $S = S-\{i_t\} \cup \{c_{1},\dots,c_{s_t}\}$. 
        \STATE Update the assignment function: $\forall j \in \Points: \phi'(j)=i_t$ set $\phi'(j)=\phi_t(j)$. 
    \ENDIF
\ENDFOR

\STATE Pick a point from each center in $S'$ so that $\forall h \in \Colors: \beta_h k \leq |S\cap \Points^h| \leq \alpha_h k$.
\end{algorithmic}
\end{algorithm}


\begin{algorithm}[h!] %https://tex.stackexchange.com/questions/56871/how-to-format-for-loop-for-printing-a-pseudo-code-listing 
    \caption{\textsc{Divide}}\label{alg:split_a_cluster_kcenter}
    \begin{algorithmic}[1]
    \STATE \textbf{Input}: Cluster $C'_t$, Number of divisions to make $s_t$.  
    \STATE \textbf{Output}: Set of $s_t$ centers $\{c_{1},\dots,c_{s_t}\}$ and an assignment function $\phi_t: C'_t \xrightarrow{} \{c_{1},\dots,c_{s_t}\}$.  
    \item[] % skip line (unnumbered) 
    \STATE Pick $s_t$ points from the cluster $C'_t$, let those points be $\{i_{1},\dots,i_{s_t}\}$. 
    \STATE Solve $LP(\{c_{1},\dots,c_{s_t}\},C'_t)$ in (\ref{lp:split_lp}) and call the solution $x^*_{cj}$. 
    \STATE Solve MaxFlowGF($x^*_{cj},\{c_{1},\dots,c_{s_t}\},C'_t,\{\beta_h,\alpha_h\}$). 
    \end{algorithmic}
\end{algorithm}

\paragraph{\textbf{LP}$(\{i_{1},\dots,i_{s_t}\},C'_t)$}: 
\begin{subequations}\label{lp:split_lp}
\begin{align}
&  \forall c \in \{c_{1},\dots,c_{s_t}\}: \sum_{j \in C'_{t}} x_{c j} \ge \frac{|C'_{t}|}{s_t} \label{constraint:equal_split} \\
&  \forall h \in \Colors, \forall c \in \{c_{1},\dots,c_{s_t}\}: \beta_h \sum_{j \in C'_{t}} x_{c j}  \leq  \sum_{j \in C'_{t} \cap \Points^h} x_{c j} \leq \alpha_h \sum_{j \in C'_{t}} x_{c j} \label{constraint:GF_constraint} \\
&  \forall j \in \Points: \sum_{c \in \{c_{1},\dots,c_{s_t}\}} x_{c j} =1  \label{constraint:assigned} \\ 
&  \forall j \in \Points , \forall c \in \{c_{1},\dots,c_{s_t}\}: x_{c j} \in [0,1] \label{constraint:fractional}
\end{align}
\end{subequations}

   
\begin{lemma}\label{lemma:gftogfds_general}
If $\min_{h \in \Colors} \beta_h \ge \frac{8(k-1)}{n}$, then the output clusters $\{C^{D}_{1},\dots,C^{D}_{s_t}\}$ (formed by $\{c_{1},\dots,c_{s_t}\}$ and $\phi_t$) from running \textsc{Divide} satisfy the following: (1) Each cluster satisfies the \GF{} constraint with an additive violation of at most 2, (2) Each cluster has at least one point from each color, i.e. $\forall h \in \Colors: |C^{D}_{\ell}|\ge 1$ and (3) Each point is assigned to a center point which was a point in the same original cluster. 
\end{lemma}
\begin{proof}
We start with the following lemma which states that $LP(\{c_{1},\dots,c_{s_t}\},C'_t)$ in (\ref{lp:split_lp}) is feasible. 
\begin{lemma}
$LP(\{c_{1},\dots,c_{s_t}\},C'_t)$ is feasible. 
\end{lemma}
\begin{proof}
We show that the LP is feasible by showing a set of possible values for $x_{cj}$ that satisfy all of the constraints of (\ref{lp:split_lp}). Let $z_{ij}$ be the assignment in cluster $C_t$, then set $x_{cj} = \frac{z_{ij}}{s_t}$. We can then show that the assignments satisfy constraints (\ref{lp:split_lp}). 
\end{proof}

\begin{lemma}
Each cluster in the output of MaxFlowGF($x^*_{cj},\{c_{1},\dots,c_{s_t}\},C'_t,\{\beta_h,\alpha_h\}$) satisfies the \GF{} constraint with an additive violation of at most 2. 
\end{lemma}
\begin{proof}
This follows by construction of the Max-Flow problem and the given LP solution $x^*_{cj}$. 
\end{proof}


\begin{lemma}
    Each cluster has at least one point from each color.  
\end{lemma}
\begin{proof}
If the cluster is not the output of the \textsc{Divide} subroutine, then it must have a point of each color since the solution $(\bs,\bphi)$ satisfies the \GF{} constraints.  

If the cluster is the output of \textsc{Divide}, then since its parent cluster was chosen then it must satisfy the following: 
\begin{align}
    |C^h_{i}| & \ge \beta_h |C_i| -2  \\ 
              & \ge \beta_h \floor{\frac{n}{\bk+t} \frac{s_i}{s_i+1}} -2  \\
              & \ge \beta_h \Big( \frac{n}{\bk+t} \frac{1}{2} -1 \Big)-2 \\
              & \ge \beta_h \frac{n}{\bk+t} \frac{1}{2} - 3 \\ 
              & \ge 4-3 = 1 
  \end{align}
\end{proof}
\begin{lemma}
Each point is assigned to a center point which was a point in the same original cluster. 
\end{lemma}
\begin{proof}
This follows since \textsc{Divide} does not choose centers from outside.
\end{proof}
\end{proof}

\begin{theorem}\label{th:gf_to_gfpds_general}
If $\min_{h \in \Colors} \beta_h \ge \frac{8(k-1)}{n}$, then given a solution $(\bs,\bphi)$ that satisfies \GF{} for the $k$-center problem with cost $\barf$, then we can obtain a solution $(S,\phi)$ that satisfies \GF{} with an additive violation of at most $2$ and \DS{} constraints simultaneously at a cost of $2\barf$ using Algorithm \ref{alg:general_gfTogfds_kcenter}. 
\end{theorem}
\begin{proof}
This follows immediately from Lemma \ref{lemma:gftogfds_general}.  
\end{proof}

\begin{corollary}
If $\min_{h \in \Colors} \beta_h \ge \frac{8(k-1)}{n}$, given an $\alpha_{\GF}$-approximation algorithm for \GF{}, then we can have a $2\alpha_{\GF}$-approximation algorithm that satisfies \GF{} at an additive violation of $2$ and \DS{} simultaneously. 
\end{corollary}





